DetoxLLM: A Framework for Detoxification with Explanations

Prior works on detoxification are scattered in the sense that they do not cover all aspects of detoxification needed in a real-world scenario. Notably, prior works restrict the task of developing detoxification models to only a seen subset of platforms, leaving the question of how the models would perform on unseen platforms unexplored. Additionally, these works do not address non-detoxifiability, a phenomenon whereby the toxic text cannot be detoxified without altering the meaning. We propose DetoxLLM, the first comprehensive end-to-end detoxification framework, which attempts to alleviate the aforementioned limitations. We first introduce a cross-platform pseudo-parallel corpus applying multi-step data processing and generation strategies leveraging ChatGPT. We then train a suite of detoxification models with our cross-platform corpus. We show that our detoxification models outperform the SoTA model trained with human-annotated parallel corpus. We further introduce explanation to promote transparency and trustworthiness. DetoxLLM additionally offers a unique paraphrase detector especially dedicated for the detoxification task to tackle the non-detoxifiable cases. Through experimental analysis, we demonstrate the effectiveness of our cross-platform corpus and the robustness of DetoxLLM against adversarial toxicity.

==> Experiments_Prev.tex <==
\subsection{Models Comparison}

\noindent \colorbox{red!30}{\textbf{SoTA Baseline.}} We compare our models with the following state-of-the-art detoxification models. We evaluate these model directly on our dataset to determine the efficacy of the model on the cross-platform detoxification task.

\noindent \textbf{ParaDetox}~\citep{logacheva-etal-2022-paradetox} is a BART-based model finetuned on crowdsourced parallel detoxification corpus. The models is trained on three platforms, namely, Jigsaw~\citep{jigsaw} (Wikipedia's talk edit page), Reddit, and Twitter (now known as X).

\noindent \textbf{ParaGeDi}~\citep{dale-etal-2021-skoltechnlp} is a GPT-2-based model that is assisted by a style-informed classifier to re-weight the output.

%\noindent \textbf{CondBERT}~\citep{dale-etal-2021-skoltechnlp} is a token-level detoxification model which employs a BERT classifier to replace the toxic tokens.

\noindent \colorbox{orange!30}{\textbf{*-DSS.}} We further compare our models with SoTA distillation method, \textit{Distilling Step-by-Step} (DSS) proposed by~\citet{dss-Hsieh}. We use DSS method to distill both detoxification and explanation coming from \texttt{ChatGPT} into BART and T5 models. Following the work, we use a multitask framework to combine the training of generating both non-toxic version and explanation from the models given a toxic input.

\noindent \colorbox{yellow!50}{\textbf{Instruction-tuned.}} We additionally evaluate the performance of generic instruction-tuned models like Alpaca~\citep{alpaca}, instruction-tuned LLaMA (Chat)~\citep{llama2}, and Vicuna~\citep{vicuna} on the cross-platform detoxification tasks. We use the 7B version for all the models. These models are already finetuned on a wide range of generic tasks. Hence, we omit these models from further finetuning on the cross-platform detoxification to evaluate the generalizability of the models.


\noindent \colorbox{blue!30}{\textbf{Cross-Platform Models.}} We finetune a suit of models on the cross-platform datasets. Especially, we finetune BART and T5 to directly compare against the contemporary SoTA (e.g., ParaDetox). We further finetune LLM like LLaMA to observe the performance of LLM as well as compare against generic instruction-tuned models (e.g., Alpaca). As discussed in Section~\ref{sec:model_training}, we finetune our models in multiple setups. For T5 and BART, we (1) direct finetune the model to generate non-toxic version given the toxic version \underline{(vanilla)}; (2) concatenate a prompt with toxic version as the model input \underline{(prompt)}; (3) employ CoT finetuning to instruct the model explain why the given input is toxic before generating the non-toxic version \underline{(CoT-expl)}. For LLaMA finetuning, we use the two variations mentioned above namely, (1) prompt and (2) CoT-expl. We provide the detail finetuning information in Appendix~\ref{appendix:implementation_details}.



\subsection{Performance Metrics}

We report the models' performance on seven unseen platforms (Table~\ref{table:result_cross_platform}) as well as the overall average performance across all the platforms. We evaluate the models based on the following metrics.

\noindent \textbf{Accuracy.} Following~\citet{logacheva-etal-2022-paradetox}, we compute the accuracy of the models based on the percentage of non-toxic outputs identified by a style classifier. We use the same RoBERTa style classifier as the authors.

\noindent \textbf{BERTScore.} We use BERTScore to compute how the models preserve the semantic meaning. Specifically, we utilize SimCSE~\citep{simcse} RoBERTa-large model to obtain the embeddings of the input-output pair and measure the similarity between them.

\noindent \textbf{Fluency.} Following~\citet{logacheva-etal-2022-paradetox}, we measure the percentage of fluent sentences identified by a RoBERTa-based classifier of linguistic acceptability trained on the CoLA dataset~\citep{cola-warstadt}.

\noindent \textbf{BLEU.} We compute the BLEU score between the generated non-toxic version and the original non-toxic version on the test set.

==> Results_Prev.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%% Table for Cross-Platform %%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{% use resizebox with textwidth
\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc|cccc|cccc}
\hline
                                                                    & \multicolumn{4}{c}{\cellcolor{red}\textbf{Overall}}                                & \multicolumn{4}{c}{\cellcolor{cyan}\textbf{yt\_reddit}}                             & \multicolumn{4}{c}{\cellcolor{green}\textbf{fb\_yt}}                                 & \multicolumn{4}{c}{\cellcolor{orange}\textbf{fox news}}                               & \multicolumn{4}{c}{\cellcolor{pink}\textbf{convai}}                                 & \multicolumn{4}{c}{\cellcolor{yellow}\textbf{gab}}                                    & \multicolumn{4}{c}{\cellcolor{magenta}\textbf{hatecheck}}                              & \multicolumn{4}{c}{\cellcolor{cyan!30}\textbf{stormfront}}                             \\ \hline 
\textbf{Model}                                                      & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    & \textbf{Acc}    & \textbf{BS}    & \textbf{Fl}     & \textbf{BL}    \\ \hline
\cellcolor{red!30}\textbf{ParaDetox}                                                  & 67.86           & \textbf{96.51} & 91.14           & 29.13          & 44.00           & \textbf{97.43} & 76.00           & 27.52          & 79.00           & 95.50          & 93.00           & 21.16          & 78.00           & \textbf{97.37} & 96.00           & 35.08          & 82.00           & \textbf{95.93} & 97.00           & 31.66          & 80.00           & 94.49          & 83.00           & 25.41          & 24.00           & \textbf{98.02} & 98.00           & 22.68          & 88.00           & \textbf{96.83} & 95.00           & 40.38          \\
\cellcolor{orange!30}\textbf{T5-DSS}                                                     & 68.33           & 95.55          & 96.72           & 38.88          & 67.39           & 95.70          & 97.83           & 35.73          & 72.41           & 95.74          & 98.85           & 41.97          & 73.63           & 95.07          & 94.51           & 38.26          & 64.84           & 95.65          & 94.51           & 38.91          & 68.89           & \textbf{95.41} & 96.67           & 40.39          & 68.09           & 95.20          & 95.74           & 38.00          & 63.04           & 96.11          & 98.91           & 38.89          \\
\cellcolor{orange!30}\textbf{BART-DSS}                                                   & 85.77           & 93.85          & 97.80           & 43.53          & 82.61           & 93.61          & 93.48           & 39.32          & 94.25           & 93.78          & 98.85           & 47.45          & 86.81           & 94.04          & 95.60           & 43.64          & 84.62           & 93.84          & 98.90           & 42.51          & 81.11           & 93.79          & 98.89           & 47.26          & 82.98           & 93.81          & \textbf{100.00} & 40.96          & 88.04           & 94.06          & 98.91           & 43.55          \\
\cellcolor{blue!30}\textbf{T5-V}     & 74.86           & 94.08          & 98.71           & 36.91          & 62.00           & 94.48          & 98.00           & 34.16          & 76.00           & \textbf{96.23} & 98.00           & 42.10          & 88.00           & 92.85          & 99.00           & 34.78          & 81.00           & 93.71          & \textbf{100.00} & 36.76          & 82.00           & 93.65          & 97.00           & 38.52          & 50.00           & 94.17          & \textbf{100.00} & 31.87          & 85.00           & 93.50          & 99.00           & 40.18          \\
\cellcolor{blue!30}\textbf{T5-P}     & 75.43           & 91.61          & 97.71           & 36.59          & 70.00           & 91.37          & 94.00           & 32.93          & 80.00           & 93.97          & 99.00           & 40.84          & 87.00           & 91.46          & 98.00           & 37.24          & 80.00           & 91.71          & 99.00           & 35.93          & 78.00           & 91.74          & 96.00           & 38.89          & 46.00           & 90.50          & 99.00           & 30.42          & 87.00           & 90.50          & 99.00           & 39.91          \\
\cellcolor{blue!30}\textbf{CE}    & 74.10           & 89.57          & 96.23           & 34.91          & 67.39           & 89.21          & 97.83           & 32.35          & 78.16           & 89.69          & 95.40           & 37.93          & 72.53           & 89.48          & 96.70           & 34.25          & 68.13           & 89.41          & 94.51           & 33.13          & 76.67           & 89.74          & 97.78           & 38.23          & 82.98           & 89.37          & 94.68           & 34.91          & 72.83           & 90.12          & 96.74           & 33.58          \\
\cellcolor{blue!30}\textbf{BART-V}   & 88.71           & 93.60          & 98.14           & 40.06          & 88.00           & 92.88          & 98.00           & 38.14          & 96.00           & 94.48          & 99.00           & 45.85          & 93.00           & 94.48          & 100.00          & 41.50          & 89.00           & 93.00          & 99.00           & 34.11          & 90.00           & 92.55          & 93.00           & 41.06          & 73.00           & 93.58          & 99.00           & 34.31          & 92.00           & 94.24          & 99.00           & 45.43          \\
\cellcolor{blue!30}\textbf{BART-P}    & 83.00           & 91.32          & 97.86           & 38.99          & 74.00           & 91.04          & 98.00           & 36.77          & 89.00           & 92.97          & 100.00          & 44.11          & 92.00           & 91.67          & 99.00           & 39.77          & 85.00           & 91.34          & 98.00           & 35.49          & 87.00           & 90.78          & 96.00           & 40.10          & 67.00           & 89.73          & 98.00           & 32.51          & 87.00           & 91.73          & 96.00           & 44.20          \\
\cellcolor{blue!30}\textbf{BART-CE}  & 87.29           & 89.23          & 98.59           & 36.78          & 80.43           & 89.27          & \textbf{100.00} & 37.39          & 89.66           & 89.34          & 100.00          & 38.58          & 89.01           & 88.91          & 96.70           & 35.76          & 89.01           & 89.24          & 97.80           & 35.62          & 85.56           & 89.30          & 98.89           & 40.96          & 90.43           & 89.01          & 98.94           & 34.63          & 86.96           & 89.54          & 97.83           & 34.55          \\ \hline
\cellcolor{yellow!50}\textbf{Alpaca}                                                     & 99.53           & 84.85          & \textbf{100.00} & 9.87           & \textcolor{gray}{\textbf{100.00}} & 84.67          & \textbf{100.00} & 12.29          & \textcolor{gray}{\textbf{100.00}} & 84.52          & \textbf{100.00} & 6.25           & 98.90           & 85.03          & \textbf{100.00} & 9.81           & 98.90           & 84.92          & \textbf{100.00} & 10.97          & 98.89           & 84.39          & \textbf{100.00} & 10.65          & \textcolor{gray}{\textbf{100.00}} & 85.81          & \textbf{100.00} & 9.91           & \textcolor{gray}{\textbf{100.00}} & 84.60          & \textbf{100.00} & 9.23           \\
\cellcolor{yellow!50}\textbf{LLaMA-C}     & \textcolor{gray}{\textbf{100.00}} & 84.74          & \textbf{100.00} & 9.60           & \textcolor{gray}{\textbf{100.00}} & 84.60          & \textbf{100.00} & 11.45          & \textcolor{gray}{\textbf{100.00}} & 84.38          & \textbf{100.00} & 6.97           & \textcolor{gray}{\textbf{100.00}} & 84.90          & \textbf{100.00} & 9.34           & \textcolor{gray}{\textbf{100.00}} & 84.70          & \textbf{100.00} & 10.03          & \textcolor{gray}{\textbf{100.00}} & 84.32          & \textbf{100.00} & 10.63          & \textcolor{gray}{\textbf{100.00}} & 85.71          & \textbf{100.00} & 9.55           & \textcolor{gray}{\textbf{100.00}} & 84.60          & \textbf{100.00} & 9.23           \\
\cellcolor{yellow!50}\textbf{Vicuna}                                                     & 90.46           & 84.92          & 99.84           & 10.72          & 93.48           & 84.94          & \textbf{100.00} & 10.69          & 94.25           & 84.78          & \textbf{100.00} & 12.58          & 87.91           & 84.93          & \textbf{100.00} & 9.72           & 91.21           & 85.07          & \textbf{100.00} & 11.98          & 91.11           & 83.69          & 98.89           & 11.97          & 89.36           & 86.28          & \textbf{100.00} & 9.72           & 85.87           & 84.77          & \textbf{100.00} & 8.40           \\ \hline
\cellcolor{blue!30}\textbf{LLaMA-P}  & 92.02           & 91.83          & 98.42           & 59.19          & 84.78           & 91.13          & 97.83           & 49.39          & 96.55           & 91.99          & 97.70           & \textbf{67.89} & 93.41           & 92.04          & 97.80           & \textbf{60.71} & 87.91           & 92.04          & 96.70           & 58.25          & 93.33           & 91.89          & \textbf{100.00} & \textbf{61.47} & 93.62           & 91.49          & 98.94           & \textbf{57.05} & \textbf{94.57}  & 92.25          & \textbf{100.00} & 59.60          \\
\cellcolor{blue!30}\textbf{LLaMa-CE} & \textbf{95.94}  & 88.22          & 98.42           & \textbf{59.33} & \textbf{97.83}  & 83.61          & 97.83           & \textbf{52.98} & \textbf{98.85}  & 86.65          & 97.70           & 67.54          & \textbf{95.60}  & 87.23          & 98.90           & 58.44          & \textbf{92.31}  & 88.80          & 97.80           & \textbf{59.96} & \textbf{97.78}  & 91.67          & 98.89           & 61.27          & \textbf{95.74}  & 89.46          & 98.94           & 54.86          & 93.48           & 90.14          & 98.91           & \textbf{60.25} \\ \hline
\end{tabular}
}
\caption{
\label{table:result_cross_platform}
Performance of the models on cross-platform datasets. \textbf{Acc} = percentage of non- toxic outputs identified by a style classifier, \textbf{BS} = BERTScore, \textbf{Fl} = Fluency, \textbf{BL} = BLEU Score. \textbf{V} = Vanilla, \textbf{P} = Prompt, \textbf{CE} = CoT-expl, \textbf{C} = Chat. \textbf{Bold} font represents the best performance for a particular metric. We separately show the accuracy of the \colorbox{yellow!50}{instruction-tuned models} in \textcolor{gray}{\textbf{Bold}} due to their inability to detoxification (Section~\ref{sec:performance_instruction_llm}).
}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%% Table for Cross-Platform %%%%%%%%%%%%


\noindent \textbf{Overview.} We present the performance of the models on cross-platform detoxification in Table~\ref{table:result_cross_platform}. We observe that LLM model LLaMA finetuned with CoT explanation achieves better accuracy and BLEU score. We also notice that instruction-tuned generalized models receive almost perfect accuracy with very low BLEU score. We discuss the reason in Section~\ref{sec:performance_instruction_llm}. Overall, our finetuned cross-platform models outperform the contemporary SoTA ParaDetox in terms of accuracy and BLEU on the cross-platform dataset. We provide samples of models' responses in Appendix~\ref{appendix:modelsgeneration_sample}.
We now present the detail discussion on the performances.


\subsection{Performance against Contemporary SoTA}

We show the performance of the contemporary models (i.e., models with similar size with SoTA) in Table~\ref{table:result_cross_platform}. We find that both of our cross-platform finetuned Bart, T5 outperform the SoTA ParaDetox on all metrics except BERTScore. The better performance of ParaDetox can be attributed to its training dataset, that frequently transform the toxic input with a minimal change (e.g., deleting the strong words)~\citep{logacheva-etal-2022-paradetox}. It is to be noted that none of the models have seen data outside Wikipedia, Reddit, and Twitter. However, our finetuned models still manage to exhibit superior performance across the unseen platforms. We also find that DSS-based models like T5-DSS and BART-DSS outperforms other models their respective variations in BLEU and BERTScore while lag behind in terms of accuracy.


\subsection{Performance against Instruction-tuned LLMs}
\label{sec:performance_instruction_llm}

We compare our models' performance against the instruction-tuned LLMs. We notice that LLaMA-chat, Alpaca, and Vicuna achieves perfect accuracy in some of the platforms. However, all of them lack in BLEU and BERTScore compared to finetuned models. This is because they prioritize more on generating non-toxic text without focusing on preserving the semantic meaning. As a consequence, they often defy the instruction of detoxifying toxic inputs and frequently tend to produce a generic statement like: \textit{I'm sorry, but I cannot fulfill this request as it contains inappropriate language}. As a result, they receive high accuracy but very low BLEU score. This incapability of detoxification by the generalized LLMs can potentially be attributed to the safety measurements imposed during the pretrainig and the consequent finetuning stages~\citep{llama2}. As a result, whenever these models observe a toxic input they tend ignore the instruction of detoxifying the given input and tend to generate a safer statement. Therefore, instruction-tuned models should not be deployed for the detoxification task without further finetuning, which also signifies the importance of training a dedicated instruction-tuned models for the detoxification task. 

\subsection{Improvement through Explainability}

Table~\ref{table:result_cross_platform} shows the performance comparison of CoT-expl and vanilla finetuned models. As evident, CoT-expl LLaMA outperforms LLaMA-prompt in terms of accuracy while the later achieves better BERTScore. We believe CoT explanation first help the models to identify the specific words or semantics that turns a text into toxic. %(Appendix XX).
As a consequence, during the style transfer process, the models can focus on removing/modifying those specific portion to alleviate toxicity. Therefore, CoT-expl helps the models to achieve better accuracy. However, identification of toxicity in an input text also means altering that input text. Hence, CoT-expl models achieves inferior BERTScore than vanilla models. Considering the nature of the detoxification task, it is more important to produce non-toxic text even that costs a few alterations of the input. Therefore, we perfer CoT-expl LLaMA models over the models in this work.

\subsection{Performance on ParaDetox}


%%%%%%%%%%%%%%%%%%%%%%%%% Table for ParaDetox %%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\tiny
\resizebox{\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{lcccc}
\hline
\textbf{Model}                                                      & \textbf{Acc}   & \textbf{BS}    & \textbf{Fl}    & \textbf{BL}    \\ \hline
\cellcolor{red!30}\textbf{ParaDetox}                                                  & 90.16          & \textbf{96.65} & 88.52          & \textbf{69.99} \\
\cellcolor{orange!30}\textbf{T5-DSS}                                                     & 87.63          & 93.78          & 96.57          & 55.98          \\
\cellcolor{orange!30}\textbf{BART-DSS}                                                   & 92.10          & 93.68          & 96.27          & 52.38          \\
\cellcolor{blue!30}\textbf{T5-V}     & 91.21          & 93.81          & 95.23          & 54.78          \\
\cellcolor{blue!30}\textbf{T5-P}      & 89.42          & 93.97          & 94.93          & 55.47          \\
\cellcolor{blue!30}\textbf{T5-CE}    & 88.23          & 94.04          & 95.38          & 56.39          \\
\cellcolor{blue!30}\textbf{BART-V}   & 92.85          & 93.28          & 96.42          & 48.80          \\
\cellcolor{blue!30}\textbf{BART-P}    & 93.59          & 93.81          & 95.68          & 53.46          \\
\cellcolor{blue!30}\textbf{BART-CE}  & 93.29          & 93.01          & 96.72          & 48.74          \\ \hline
\cellcolor{yellow!50}\textbf{Alpaca}                                                     & 71.39          & 95.22          & 95.23          & 62.46          \\
\cellcolor{yellow!50}\textbf{LLaMA-C}     & \textcolor{gray}{\textbf{94.63}} & 92.08          & 97.47          & 43.34          \\
\cellcolor{yellow!50}\textbf{Vicuna}                                                     & 79.73          & 93.72          & \textbf{98.06} & 53.26          \\ \hline
\cellcolor{blue!30}\textbf{LLaMA-P}  & 93.89          & 92.72          & \textbf{98.06} & 42.55          \\
\cellcolor{blue!30}\textbf{LLaMA-CE} & \textbf{94.04} & 92.51          & 97.47          & 41.22          \\ \hline
\end{tabular}
}
\caption{
\label{table:result_paradetox}
Performance of the models on human annotated ParaDetox test set. \textbf{Acc} = percentage of non- toxic outputs identified by a style classifier, \textbf{BS} = BERTScore, \textbf{Fl} = Fluency, \textbf{BL} = BLEU Score. \textbf{V} = Vanilla, \textbf{P} = Prompt, \textbf{CE} = CoT-expl, \textbf{C} = Chat. \textbf{Bold} font represents the best performance for a particular metric. We separately show the accuracy of the \colorbox{yellow!50}{instruction-tuned models} in \textcolor{gray}{\textbf{Bold}} due to their inability to detoxification (Section~\ref{sec:performance_instruction_llm}).
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%% Table for ParaDetox %%%%%%%%%%%%

We further compare the models' performance against the human annotated parallel data. For this purpose, we evaluate the models on the test set of ParaDetox. As Table~\ref{table:result_paradetox} shows, ParaDetox achieves the best BERTScore and BLEU on this test set, which is unsurprising since the model has already been trained on this dataset. Noticeably, our suit of cross-platform models still shows comparable BERTScore, while even outperforming ParaDetox in terms of accuracy and fluency. This result implicates two important dimensions: \textbf{(1)} Although our dataset is artificially generated, the models trained on this dataset shows impressive performance on human-annotated dataset. This signifies the usability of our dataset. \textbf{(2)} Our models are trained on the same platforms as ParaDetox, but the parallel data are completely different. Hence, the performance of our models indicates the better generalization capability.


\subsection{Paraphrase Detection}


%%%%%%%%%%%%%%%%%%%%%%%%% Table for Paraphrase %%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
%\tiny
\resizebox{\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{lcc}
\hline
\textbf{Model} & \textbf{Accuracy} & \textbf{F\textsubscript{1}-score} \\ \hline
BERT~\citep{bert}     & 79.33                & 80.88          \\
RoBERTa~\citep{roberta}           & 76.42                & 77.39          \\
ELECTRA~\citep{electra}        & 35.52                & 16.12          \\
TextAttack-BERT~\citep{textattack}        & 34.55                & 29.21          \\
TextAttack-RoBERTa~\citep{textattack}        & 28.96                & 13.61          \\
Sentence-BERT~\citep{sentence-bert}        & 50.00                & 66.63          \\
BERT \textbf{(ours)}    & \textbf{85.73}                & \textbf{86.13}          \\ \hline
\end{tabular}
}
\caption{
\label{table:performance_paraphrase}
Performance of the models on the paraphrase detection task. We compare our model's performance against SoTA baselines finetuned on MRPC~\citep{mrpc} dataset. \textbf{Bold} font represents the best performance for a particular metric.
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%% Table for Paraphrase %%%%%%%%%%%%


We test the paraphrase detection capability of our finetuned BERT by passing a set of detoxifiable and non-detoxifiable texts. For this purpose, we sample human-annotated parallel data (detoxifiable) from ParaDetox~\citep{logacheva-etal-2022-paradetox}. We also sample the human-labeled non-detoxifiable toxic data from ParaDetox and generate the corresponding non-toxic version with our finetuned detoxification model. Since the toxic set cannot be detoxified by human, we consider these toxic, non-toxic pairs as non-detoxifiable. We expect the paraphrase detection model to produce positive for detoxifiable and negative for non-detoxifiable texts so that our framework can warn the users in case meaning alteration. We situate our model's performance against SoTA baselines finetuned on MRPC~\citep{mrpc} paraphrase detection task.

We present the result in Table~\ref{table:performance_paraphrase}. As evident, our paraphrase detector conveniently outperforms the SoTA baselines. This shows the importance of a dedicated paraphrase detector in our framework, since the models trained on generic paraphrase benchmark are unable to transfer their knowledge when understanding the semantic meaning between toxic / non-toxic pairs.

==> table_human_annotator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\renewcommand*{\arraystretch}{1.2}   %to squeeze table content
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccccccccc}
\hline
\multirow{2}{*}{\textbf{Evaluator}} & \multicolumn{6}{c}{\textbf{ParaDetox}} & \textbf{} & \multicolumn{6}{c}{\textbf{BART-V (ours)}} & \textbf{} & \multicolumn{6}{c}{\textbf{\textbackslash{}xdetox (ours)}} \\ \cline{2-7} \cline{9-14} \cline{16-21} 
                                    & A      & B     & C  & D  & N-A  & N-D  &           & A   & B   & C     & D      & N-A   & N-D   &           & A       & B        & C      & D        & N-A     & N-D     \\ \hline
1                                   & 42     & 6     & 0  & 2  & a    & b    &           & 2   & 2   & 1     & 45     & aa    & bb    &           & 43      & 0        & 0      & 7        & aaa     & bbb     \\
2                                   & 45     & 3     & 0  & 2  & c    & d    &           & 4   & 0   & 2     & 44     & cc    & dd    &           & 41      & 7        & 2      & 0        & ccc     & ddd     \\
3                                   & 45     & 3     & 0  & 2  & e    & f    &           & 4   & 0   & 2     & 44     & ee    & ff    &           & 41      & 7        & 2      & 0        & eee     & fff     \\
4                                   & 45     & 3     & 0  & 2  & g    & h    &           & 4   & 0   & 2     & 44     & gg    & hh    &           & 41      & 7        & 2      & 0        & ggg     & hhh     \\
Avg                                 & 43.5   & 4.5   & 0  & 2  & i    & j    &           & 3   & 1   & 1.5   & 44.5   & ii    & jj    &           & 42      & 3.5      & 1      & 43.5     & iii     & jjj     \\
Sum                                 & 87     & 9     & 0  & 4  & k    & l    &           & 6   & 2   & 3     & 89     & kk    & ll    &           & 84      & 7        & 2      & 7        & kkk     & lll     \\ \hline
\end{tabular}
}
\caption{\label{table:human-evaluation-result}
Detail human evaluation result. 
}
\end{table*}

